Unsupervised Meta-Learning For Few-Shot Image Classification

Few-shot or one-shot learning of classifiers requires a significant inductive bias towards the type of task to be learned. One way to acquire this is by meta-learning on tasks similar to the target task. In this paper, we propose UMTRA, an algorithm that performs unsupervised, model-agnostic meta-learning for classification tasks. The meta-learning step of UMTRA is performed on a flat collection of unlabeled images. While we assume that these images can be grouped into a diverse set of classes and are relevant to the target task, no explicit information about the classes or any labels are needed. UMTRA uses random sampling and augmentation to create synthetic training tasks for meta-learning phase. Labels are only needed at the final target task learning step, and they can be as little as one sample per class. On the Omniglot and Mini-Imagenet few-shot learning benchmarks, UMTRA outperforms every tested approach based on unsupervised learning of representations, while alternating for the best performance with the recent CACTUs algorithm. Compared to supervised model-agnostic meta-learning approaches, UMTRA trades off some classification accuracy for a reduction in the required labels of several orders of magnitude.

==> sections/ExpCeleba.tex <==
\subsection{UMTRA on the CelebA dataset}
% (Siavash: Please read this section and fix grammatical and other errors)


\begin{table}
    \centering
    {\footnotesize
    \begin{tabular}{|p{2.7cm}|c|c|c|}
         \hline 
         {\bf Algorithm (N, K)} & {\bf (5, 1)} & {\bf (5, 5)} & {\bf (5, 10)}
         \\
         \hline
         {\em Training from scratch} & 26.86 & 39.65 &  50.61 
         \\
         \hline
         UMTRA (ours) & {\bf 33.43} & {\bf 50.19} & {\bf 58.84}
         \\
         \hline
         Supervised MAML & 72.26 & 84.90 & 88.26
         \\
         \hline
    \end{tabular}
    }
    \vspace{1mm}
    \caption{Comparison between our method and supervised meta-learning on CelebA dataset.}
    %The task is 5-way classification. K stands for the number of shots from each person for training. First row shows the results if we start from random initialized weights.}
    \label{tab:Celeba}
\end{table}

In this series of experiments we evaluate our algorithm on the CelebA large scale face dataset~\cite{liu2015faceattributes}. Each subject has  a different number of face images. This makes the unlabeled dataset $\mathcal{U}$ also unbalanced, a less favorable but possibly more realistic scenario. The evaluation is done on 600 different tasks, on faces whose identities were never seen during the meta-learning phase. The augmentation function was auto augment which gave the best results for Mini-Imagenet. Figure~\ref{fig:AugmentedCelebA} compares a sampled task generated by UMTRA with one of the sampled tasks generated by supervised MAML. The comparison between UMTRA, training from scratch and supervised MAML is shown in Table~\ref{tab:Celeba}.  The results confirm the trend that UMTRA outperforms learning from scratch, but performs worse than supervised learning. 

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{images/augmentation/CelebaAugmentation.pdf}
    \caption{Visualization of 5-way classification tasks generated by UMTRA (Left) and MAML (Right) on CelebA faces. Top: Task's training images. Bottom: Task's validation images.}
    \label{fig:AugmentedCelebA}
\end{figure}

% The proposed task is to identify N people based on just K images of each one of them.
%The similarity between faces. The results are based on flipping the images and translating them. UMTRA again is better than training from scratch.



==> sections/ExpUCF101.tex <==
\subsection{UMTRA for video action recognition}

% (Siavash) Ask Dr. Shah, should I remove this paragraph?

% Sports are typically, the one which can be learned easily due to distinctive motion information at each particular sport.
% Human-Object interaction clips, on the other hand, have a highly cluttered background and the motion information is not that much distinctive which make them the hardest ones to learn.
% \cite{soomro2012ucf101}

In this section, we show how the UMTRA can be applied to video action recognition, a domain significantly more complex and data intensive than the one used in the few-shot learning benchmarks such as Omniglot and Mini-Imagenet. To the best of our knowledge, we are the first to apply meta-learning to video action recognition. We perform our comparisons using one of the standard video action recognition datasets, UCF-101\cite{soomro2012ucf101}.  UCF-101 includes 101 action classes divided into five types: Human-Object Interaction, Body-Motion Only, Human Human Interaction, Playing Musical Instruments and Sports. The dataset is composed of snippets of Youtube videos. Many videos have poor lighting, cluttered background and severe camera motion. As the classifier on which to apply the meta-learning process, we use a 3D convolution network, C3D~\cite{tran2015learning}.

Performing unsupervised meta-learning on video data, requires several adjustments to the UMTRA workflow, with regards to the initialization of the classifier, the split between meta-learning data and testing data, and the augmentation function. 

First, networks of the complexity of C3D cannot be learned from scratch using the limited amount of data available in few-shot learning. In the video action recognition research, it is common practice to start with a network that had been pre-trained on a large dataset, such as Sports-1M dataset~\cite{karpathy2014large}, an approach we also use in all our experiments. 

Second, we make the choice to use two different datasets for the meta-learning phase (Kinetics~\cite{tran2015learning, jia2014caffe, KarpathyCVPR14}) and for the few-shot learning and evaluation (UCF-101~\cite{soomro2012ucf101}). This gives us a larger dataset for training since Kinetics contains 400 action classes, but it introduces an additional challenge of domain-shift: the network is pre-trained on Sports-1M, meta-trained on Kinetics and few-shot trained on UCF-101. This approach, however, closely resembles the practical setup when we need to do few-shot learning on a novel domain. When using the Kinetics dataset for meta-learning, we limit it to 20 instances per class.

For the augmentation function $\mathcal{A}$, working in the video domain opens a new possibility, of creating an augmented sample by choosing a temporally shifted video fragment from the same video. Figure \ref{fig:AugmentedKinetics} shows some samples of these augmentations. In our experiments, we have experimented both with UMTRA (using a Kinetics dataset stripped from labels), and supervised meta-learning (retaining the labels on Kinetics for the choice of the validation, but following the rest of the experimental protocol). This supervised meta-learning experiment is also significant because, to the best of our knowledge, meta-learning has never been applied to human action recognition from videos. 

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{images/augmentation/VideoAugmentation.pdf}
    \caption{Example of the training data and the augmentation function $\mathcal{A}$ for video. The training data $x$ is a 16 frame segment starting from a random time in the video sample (Here we show three frames of a sample at each column). The validation data $x' = \mathcal{A}(x)$ is also a 16 frame segment, starting from a different, randomly selected time {\em from the same video sample}.}
    \label{fig:AugmentedKinetics}
\end{figure}

In our evaluation, we perform 30 different experiments. At each experiment we sample 5 classes from UCF-101, perform the one-shot learning, and evaluate the classifier on all the examples for the 5 classes from UCF-101. As the number of samples per class are not the same for all classes, in  Table~\ref{tab:UCF101-Results} we report both the accuracy and F1-score.

The results allow us to draw several conclusions. The relative accuracy ranking between training from scratch, pre-training and unsupervised meta-learning and supervised meta-learning remained unchanged. Supervised meta-learning had proven feasible for one-shot classifier training for video action recognition. UMTRA performs better than other approaches that use unsupervised data. Finally, we found that the domain shift from Kinetics to UCF-101 was successful. 

\begin{table}
    \centering
    {\footnotesize
    \begin{tabular}{|p{4.25cm}|p{3cm}|}
    \hline
    {\bf Algorithm} & {\bf Test Accuracy / F1-Score} \\
        \hline 
        {\em Training from scratch} & 29.30 / 20.48\\
        \hline
        Pre-trained on Kinetics & 45.51 / 42.49\\ 
        \hline
        UMTRA on unlabeled Kinetics (ours) & \textbf{60.33 / 58.47}\\
        \hline
        Supervised MAML on Kinetics & 71.08 / 69.44\\
        \hline
        \end{tabular}
    }
    \vspace{1mm}
    \caption{Accuracy and F1-Score for a 5-way, one-shot classifier trained and evaluated on classes sampled from UCF-101. All training (even for ``training from scratch''), employ a C3D network pre-trained on Sports-1M. For all approaches, none of the UCF-101 classes was seen during pre- or meta-learning.}
    \label{tab:UCF101-Results}
\end{table}


% \begin{figure}
%     \centering
%     \includegraphics[width=2cm]{images/train-cello.png} 
%     \hspace{4pt}
%     \includegraphics[width=2cm]{images/validation_cello.png}
%     \vspace{4pt}
%     \includegraphics[width=2cm]{images/train_climbing.png}
%     \hspace{4pt}
%     \includegraphics[width=2cm]{images/validation_climbing.png}
%     \caption{Some samples of clips used for meta training. The left images are frames from the clips which are used for training set and the right images are frames from the clips which are used for validation. The variation between examples are much more than characters. Actions: Playing cello and Wall Climbing}
%     \label{fig:UCF101-MetaTraining}
% \end{figure}


% \begin{table}
%     \centering
%     {\footnotesize
%     \begin{tabular}{|p{1.3cm}|p{0.9cm}|p{0.9cm}|p{0.9cm}|p{0.8cm}|p{0.8cm}|}
%     \hline
%     & Billiards & Hand-stand Pushups & Parallel Bars & Playing Dhol & Shotput \\ 
%     \hline
%     Billiards & 138 & 0 & 0 & 0 & 0 \\
%     \hline
%     Handstand Pushups & 6 & 110 & 10 & 20 & 0 \\
%     \hline
%     Parallel Bars & 2 & 2 & 49 & 6 & 0 \\
%     \hline
%     Playing Dhol & 2 & 1 & 24 & 110 & 0 \\
%     \hline
%     Shotput & 2 & 7 & 31 & 28 & 114 \\
%     \hline
%     Accuracy & 92\% & 91.66\% & 42.98\% & 67.97\% & 100\% \\
%     \hline
%     \end{tabular}
%     }
%     \caption{Confusion Matrix for the 5-way classification task which gave the best results. UCF-101 Training on 5-way 1-shot}
%     \label{tab:best_task_ucf101}
% \end{table}


% \begin{table}
%     \centering
%     {\footnotesize
%     \begin{tabular}{|p{1.3cm}|p{0.9cm}|p{0.9cm}|p{0.9cm}|p{0.8cm}|p{0.8cm}|}
%     \hline
%     & Diving & Playing Daf & Playing Flute & Sky-diving & Surfing \\
%     \hline
%     Diving & 0 & 0 & 0 & 0 & 0 \\
%     \hline
%     Playing Daf & 75 & 6 & 1 & 5 & 0 \\
%     \hline
%     Playing Flute & 7 & 145 & 151 & 1 & 0 \\
%     \hline
%     Skydiving & 28 & 0 & 2 & 101 & 54 \\
%     \hline
%     Surfing & 37 & 0 & 1 & 1 & 72 \\
%     \hline
%     \end{tabular}
%     }
%     \caption{Worst Task Confusion Matrix for UCF-101 Training on 5-way 1-shot}
%     \label{tab:worst_task_ucf101}
% \end{table}


% \begin{figure}
%     \centering
%     \includegraphics[width=2cm,height=2cm,keepaspectratio]{images/worst_actions1.png} 
%     \includegraphics[width=2cm,height=2cm,keepaspectratio]{images/worst_actions2.png} 
%     \includegraphics[width=2cm,height=2cm,keepaspectratio]{images/worst_actions3.png} 
    
%     \includegraphics[width=2cm,height=2cm,keepaspectratio]{images/worst_actions4.png} 
%     \includegraphics[width=2cm,height=2cm,keepaspectratio]{images/worst_actions5.png} 
    
%     \caption{The only action clips which were used for the task of classifying these actions. Action classes are SkyDiving, Playing Flute, Diving, Surfing and PlayingDaf.}
%     \label{fig:pocessing_images}
% \end{figure}

==> sections/ExperimentsImages.tex <==
\subsection{Result on Image Datasets}

Omniglot~\cite{lake2011one} is a dataset of handwritten characters frequently used to compare few-shot learning algorithms. It comprises 1623 characters from 50 different alphabets. Every character in Omniglot has 20 different instances each was written by a different person. To allow comparisons with other published results, in our experiments we follow the experimental protocol described in \cite{santoro2016meta}: 1200 characters were used for training and 423 characters were used for testing. 

UMTRA, like the supervised MAML algorithm is model-agnostic, that is, it does not impose conditions on the actual network architecture used in the learning. This does not, of course, mean that the algorithm performs identically for every network structure and dataset. In order to separate the performance of the architecture and the meta-learner, we run our experiments using an architecture originally proposed in~\cite{vinyals2016matching}. This classifier uses four 3 x 3 convolutional modules with 64 filters each, followed by batch normalization~\cite{ioffe2015batch}, a ReLU nonlinearity and 2 x 2 max-pooling. On the resulting feature embedding, the classifier is implemented as a fully connected layer followed by a softmax layer. 

%In order to investigate whether the classifier architecture makes a difference in the implementation structure, we have also run some experiments with a different al

The first question is what type of augmentation functions and hyperparameter settings we should use? UMTRA has a relatively large hyperparameter space that includes the augmentation function. As pointed out in a recent study involving performance comparisons in semi-supervised systems~\cite{oliver2018realistic}, excessive tuning of hyper-parameters can easily lead to an overestimation of the performance of an approach compared to simpler approaches. Thus, for the comparison in the reminder of this paper, we keep a relatively small budget for hyperparameter search: beyond basic sanity checks we only tested 5-10 hyperparameter combinations per dataset, without specializing them to the N or K parameters of the target task. Table~\ref{tab:AugmentationCompare} shows several choices for the augmentation function for the 5-way one-shot classification in Omniglot. Based on this table, in comparing with other approaches, we use an augmentation function consisting of randomly zeroed pixels and random shift.

% As a note, based on the spread of the accuracies in Table~\ref{tab:AugmentationCompare}, it is very likely that other choices of hyperparameters, possibly specialized to the $N$ and $K$ values may offer higher accuracy values. Depending on the needs of an application and the computational budget available, in practice it may be worthwhile to perform such a hyperparameter search step. This however, is beyond the scope of this paper. 


\begin{table}
    \centering
    {\footnotesize
    %\begin{tabular}{|p{5cm}|p{1cm}|}
    \begin{tabular}{|p{6cm}|p{2cm}|}
         \hline 
         {\bf Augmentation Function $\mathcal{A}$} & 
        %  {\bf Meta-batch size $N_\mathit{MB}$} &
        % {\bf No. of\newline updates $N_U$} &
         {\bf Accuracy} \\
         \hline
         {\em Training from scratch} &
        %   N/A & 
        %   N/A &
         52.50 \\
         \hline
         $\mathcal{A} = \mathbbm{1}$ & 
        %   1 & 
        %   1 & 
         52.93 \\ 
         \hline
         $\mathcal{A}$ = randomly zeroed pixels & 
        %   1 & 
        %   1 &
         56.23 \\
         \hline
        $\mathcal{A}$ = 
         randomly zeroed pixels 
         \newline $~~~~~\quad$
        + random shift & 
        %  1 & 1 & 
        67.08 \\
         \hline
         $\mathcal{A}$ = randomly zeroed pixels 
          \newline $~~~~~\quad$
        + random shift (with best hyper parameters) & 
        %   25 & 10 & 
         \textbf{83.26} \\
         \hline
         {\em Supervised MAML} & 
         98.7 \\
         \hline
    \end{tabular}
    }
    \caption{The influence of augmentation function on the accuracy of UMTRA for 5-way one-shot classification on the Omniglot dataset.}
    \label{tab:AugmentationCompare}
\end{table}


\SK{
Two important hyper-parameters in meta-learning are meta batch size, $N_{MB}$, and number of updates, $N_{U}$. In table \ref{tab:hyperparameter-compare-omniglot}, we study the effect of these hyperparameters on the accuracy of the network for the randomly zerod pixels and random shift augmentation. 
}
\begin{table}
    \centering
    {\footnotesize
        \begin{tabular}{c|p{0.6cm}|p{0.6cm}|p{0.6cm}|p{0.6cm}|p{0.6cm}|p{0.6cm}}
        \diagbox{\scriptsize{$\#$ Updates}}{\scriptsize{$N_{MB}$}} & 1 & 2 & 4 & 8 & 16 & 25 \\
        \hline
        1 & 67.08 & 79.04 & 80.72 & 81.60 & 82.72 & 83.80 \\
        \hline
        5 & 76.08 & 76.68 & 77.20 & 79.56 & 81.12 & 83.32 \\
        \hline
        10 & 79.20 & 79.24 & 80.92 & 80.68 & 83.52 & 83.26\\
        \end{tabular}
    }
    \caption{The effect of hyper parameters meta batch size, $N_{MB}$, and number of updates, $N_{U}$ on accuracy.}
    \label{tab:hyperparameter-compare-omniglot}
\end{table}

The second consideration is what sort of baseline we should use when evaluating our approach on a few-shot learning task? Clearly, supervised meta-learning approaches such as an original MAML~\cite{finn2017model} are expected to outperform our approach, as they use a labeled training set. A simple baseline is to use the same network architecture being trained from scratch with only the final few-shot labeled set. If our algorithm takes advantage of the unsupervised training set $\mathcal{U}$, as expected, it should outperform this baseline. 

A more competitive comparison is against networks that are first trained to obtain a favorable embedding using unsupervised learning on $\mathcal{U}$, with the resulting embedding used on the few-shot learning task. While it is not a meta-learning, we can train this model with the same target task training set as UMTRA. Similar to~\cite{hsu2018unsupervised}, we compare the following unsupervised pre-training approaches: ACAI~\cite{berthelot2018understanding}, BiGAN~\cite{donahue2016adversarial}, DeepCluster~\cite{caron2018deep} and InfoGAN~\cite{chen2016infogan}. These up-to-date approaches cover a wide range of the recent advances in the area of unsupervised feature learning. Finally, we also compare against the CACTUs unsupervised meta-learning algorithm proposed in the \cite{hsu2018unsupervised}, combined with MAML and ProtoNets~\cite{snell2017prototypical}. 


Table~\ref{tab:ResultsOmniglot} shows the results of the experiments. For the UMTRA approach we trained for 6000 meta-iterations for the 5-way, and 36,000 meta-iterations for the 20-way classifications. Our approach, with the proposed hyperparameter settings outperforms, with large margins, training from scratch and the approaches based on unsupervised representation learning. UMTRA also outperforms, with a smaller margin, the CACTUs approach on all metrics, and in combination with both MAML and ProtoNets. 

As expected, the supervised meta-learning baselines perform better than UMTRA. To put this value in perspective, we need to take into consideration the vast difference in the number of labels needed for these approaches. In one-shot 5-way classification, UMTRA obtains a 77.80\% accuracy with only 5 labels, while supervised MAML obtains 94.46\% but requires 24005 labels. For 5-shot 5-way classification UMTRA obtains a 92.74\% accuracy with only 25 labels, while supervised MAML obtains 98.83\% with 24025. 

%UMTRA-mod  with additional FC layer 2000 iterations (ours).

\begin{table}
    \centering
    {\footnotesize
    \begin{tabular}{|p{3.5cm}|c|c|c|c|}
        \hline
        {\bf Algorithm (N, K)} & {\bf (5, 1)} & {\bf (5, 5)} & \bf{(20, 1)} & \bf{(20, 5)} \\
        \hline
        {\em Training from scratch} & 52.50 & 74.78 & 24.91 & 47.62 \\
        \hline
        BiGAN $k_{nn}$-nearest neighbors & 49.55 & 68.06  & 27.37 & 46.70\\
        BiGAN linear classifier & 48.28 & 68.72  & 27.80 & 45.82\\
        BiGAN MLP with dropout & 40.54 & 62.56  & 19.92 & 40.71\\
        BiGAN cluster matching & 43.96 & 58.62  & 21.54 & 31.06 \\
        BiGAN CACTUs-MAML & 58.18 & 78.66  & 35.56 & 58.62 \\
        BiGAN CACTUs-ProtoNets & 54.74 & 71.69  & 33.40 &  50.62\\
        % Siavash, please leave it like this
        % &&&&\\
        ACAI $k_{nn}$-nearest neighbors & 57.46 & 81.16 & 39.73 & 66.38 \\
        ACAI linear classifier & 61.08 & 81.82  &  43.20 & 66.33\\
        ACAI MLP with dropout & 51.95 & 77.20  &  30.65 & 58.62 \\
        ACAI cluster matching & 54.94 & 71.09  & 32.19 &  45.93 \\
        %\hline
        ACAI CACTUs-MAML & 68.84 &  87.78  & 48.09 & 73.36 \\
        ACAI CACTUs-ProtoNets & 68.12 & 83.58  & 47.75 & 66.27 \\
        % Siavash, please leave it like this
        % &&&&\\
        \hline
        UMTRA (ours) & \textbf{77.80} & \textbf{92.74} & \textbf{62.20} & \textbf{77.50} \\
        % UMTRA (ours) altern. arch. & \textbf{80.16} & \textbf{90.68} & \textbf{50.89} & \textbf{77.93} \\
        \hline
        {\em Supervised MAML (control)} & 94.46 & 98.83 &  84.60 &  96.29\\
        {\em Supervised ProtoNets (control)} & 98.35 & 99.58  & 95.31 & 98.81 \\
        \hline
        \end{tabular}
    }
    \caption{Accuracy in \% of N-way K-shot (N,K) learning methods on the Omniglot dataset. The source of values, other than UMTRA is from~\cite{hsu2018unsupervised}.}
    \label{tab:ResultsOmniglot}
\end{table}


==> sections/NotIncluded.tex <==



% Decomposition formulas

% Formally, we want the expected value of our estimation of generalization error to be equal to expected value of the 

% % However, in meta-learning we use validation error and backpropagate it through the model to learn adaptation to the task. In fact, at each iteration we are looking for estimation of the error on the task on a number of points.
% % This error will be backpropagated to update the outer $\theta$ parameters of the model.

% Based on regularization theory~\cite{girosi1995regularization}, we know that there is noise, $\epsilon$, in our observations which means that $y = f_{task} + \epsilon$, where $\epsilon \sim \mathcal{N}(0, \sigma)$.
% % Let us consider the loss on one of a given sample, $x_{0}, y_{0}$ from the task. We know
% % $\mathcal{L}(y_{0}, {f}_{\theta'}(x_{0})) = - (y \log(\hat{y}) + (1 - y) \log(1 - \hat{y})) $
% % Among all possible solutions, we are looking for the solution which will minimize $E[(y_{0} - f_{\theta'}(x_{0}))^2]$ for any given sample $(x_{0}, y_{0})$ from our task. The goal of MAML is to backpropagate a true estimation of this error to the initial parameters such that they will adapt to the solution with more generality.
% Now considering the assumption we made and our loss function, we can derive our estimation based on point $(x_{0}, y_{0})$ as follows:

% \begin{equation}
% {\centering
% \begin{split}
% E[{\mathcal{L}(y_{0}, f_{\theta'}(x_{0}))}] = E\left[\sum_{c=1}^{n}{-(y_{0})_{c}\log (f_{\theta'}(x_{0}))_{c}}\right] = -E[\sum_{c=1}^{n}{(y_{0})_{c}\log (f_{\theta'}(x_{0}))_{c}}]        \\
% = - \sum_{c=1}^{n} {E\left[(y_{0})_{c}\log (f_{\theta'}(x_{0}))_{c}\right]} 
% = - \sum_{c=1}^{n} {E[(f_{task}(x_{0}) + \epsilon_{0})_{c}\log (f_{\theta'}(x_{0}))_{c}]}\\    
% = - \sum_{c=1}^{n} {E[(f_{task}(x_{0}))_{c}\log (f_{\theta'}(x_{0}))_{c} + (\epsilon_{0})_{c}\log (f_{\theta'}(x_{0}))_{c}]}\\
% = - \sum_{c=1}^{n} {(E[(f_{task}(x_{0}))_{c}\log (f_{\theta'}(x_{0}))_{c}] + E[(\epsilon_{0})_{c}\log (f_{\theta'}(x_{0}))_{c}])}\\    
% = - (E[\sum_{c=1}^{n}{(f_{task}(x_{0}))_{c}\log (f_{\theta'}(x_{0}))_{c}}] - \sum_{c=1}^{n}{E[(\epsilon_{0})_{c}\log (f_{\theta'}(x_{0}))_{c}])}\\    
% = \textit{True Estimation of Cross Entropy} - \sum_{c=1}^{n}{E[(\epsilon_{0})_{c}\log (f_{\theta'}(x_{0}))_{c}])}\\    
% \end{split}
% }
% \end{equation}

% Let us consider the term $\sum_{c=1}^{n}{E[(\epsilon_{0})_{c}\log (f_{\theta'}(x_{0}))_{c}])}$. 
% Based on Stein's lemma, we have $E[(x~-~\mu)~\cdot~g(x)]~=~\sigma^2~E[g'(x)],$
% for a normally distributed variable $x \sim \mathcal{N}(\mu, \sigma)$ we can consider $\epsilon_{0}$ as x and we have:
% \begin{equation}
% \sum_{c=1}^{n}{E\left[(\epsilon_{0})_{c}\log (f_{\theta'}(x_{0}))_{c}\right])} = \sum_{c=1}^{n}{\sigma^2 E\left[\frac{\partial \log( (f_{\theta'}(x_{0}))_{c})}{\partial {\epsilon}_{0}}\right]}    
% \end{equation}


